Modeling bias in decision-making attractor networks

Attractor neural network models of cortical decision-making circuits represent them as dynamical systems in the state space of neural firing rates with the attractors of the network encoding possible decisions. While the attractors of these models are well studied, far less attention is paid to the basins of attraction even though their sizes can be said to encode the biases towards the corresponding decisions. The parameters of an attractor network control both the attractors and the basins of attraction. However, findings in behavioral economics suggest that the framing of a decision-making task can affect preferences even when the same choices are being offered. This suggests that the circuit encodes both choices and biases separately, that preferences can be changed without disrupting the encoding of the choices themselves. In the context of attractor networks, this would mean that the parameters can be adjusted to reshape the basins of attraction without changing the attractors themselves. How can this be realized and how do the parameters shape decision-making biases? In this PhD thesis we study this question mathematically in the context of threshold linear networks, a common firing rate model used in computational neuroscience. (Note: This is an abbreviated abstract. Please see the document for the full abstract.)

==> SupplementaryMaterial/ListOfSymbols.tex <==
% Place the list of symbols below.
\begin{eqlist}[\def\makelabel#1{\hfill#1}\labelsep 1em]

\item[$\alpha$]
The first greek letter, p.~\pageref{ChX-figure: FigureLabel3}

\item[$\alpha$]
The first greek letter, p.~\pageref{ChX-figure: FigureLabel3}

\item[$\alpha$]
The first greek letter, but we should really add some more text, though we need it to go on two lines, p.~\pageref{ChX-figure: FigureLabel7}

\item[$\alpha$]
The first greek letter, p.~\pageref{ChX-figure: FigureLabel3}

\item[$\alpha$]
The first greek letter, p.~\pageref{ChX-figure: FigureLabel4}

\item[$\alpha$]
The first greek letter, p.~\pageref{ChX-figure: FigureLabel5}

\item[$\alpha$]
The first greek letter, p.~\pageref{ChX-figure: FigureLabel6}

\item[$\alpha$]
The first greek letter, p.~\pageref{ChX-figure: FigureLabel7}

\item[$\alpha$]
The first greek letter, p.~\pageref{ChX-figure: FigureLabel8}

\item[$\alpha$]
The first greek letter, p.~\pageref{ChX-figure: FigureLabel9}

\item[$\alpha$]
The first greek letter, p.~\pageref{ChX-figure: FigureLabel10}

\item[$\alpha$]
The first greek letter, p.~\pageref{ChX-figure: FigureLabel3}

\item[$\alpha$]
The first greek letter, p.~\pageref{ChX-figure: FigureLabel4}

\item[$\alpha$]
The first greek letter, p.~\pageref{ChX-figure: FigureLabel5}

\item[$\alpha$]
The first greek letter, p.~\pageref{ChX-figure: FigureLabel6}

\item[$\alpha$]
The first greek letter, p.~\pageref{ChX-figure: FigureLabel7}

\item[$\alpha$]
The first greek letter, p.~\pageref{ChX-figure: FigureLabel8}

\item[$\alpha$]
The first greek letter, p.~\pageref{ChX-figure: FigureLabel3}

\item[$\alpha$]
The first greek letter, p.~\pageref{ChX-figure: FigureLabel3}

\item[$\alpha$]
The first greek letter, p.~\pageref{ChX-figure: FigureLabel3}

\item[$\alpha$]
The first greek letter, p.~\pageref{ChX-figure: FigureLabel3}

\item[$\alpha$]
The first greek letter, p.~\pageref{ChX-figure: FigureLabel3}

\item[$\alpha$]
The first greek letter, p.~\pageref{ChX-figure: FigureLabel3}

\item[$\alpha$]
The first greek letter, p.~\pageref{ChX-figure: FigureLabel3}

\end{eqlist}

==> SupplementaryMaterial/UserDefinedCommands.tex <==
% Place user-defined commands below.

% Define the \acro command.
\makeatletter
\newif\ifFirstPar       \FirstParfalse
\def\smc{\sc}
\def\ninepoint{\small}
\DeclareRobustCommand\SMC{%
  \ifx\@currsize\normalsize\small\else
   \ifx\@currsize\small\footnotesize\else
    \ifx\@currsize\footnotesize\scriptsize\else
     \ifx\@currsize\large\normalsize\else
      \ifx\@currsize\Large\large\else
       \ifx\@currsize\LARGE\Large\else
        \ifx\@currsize\scriptsize\tiny\else
         \ifx\@currsize\tiny\tiny\else
          \ifx\@currsize\huge\LARGE\else
           \ifx\@currsize\Huge\huge\else
            \small\SMC@unknown@warning
 \fi\fi\fi\fi\fi\fi\fi\fi\fi\fi
}
\newcommand\SMC@unknown@warning{\TBWarning{\string\SMC: unrecognised
    text font size command -- using \string\small}}
\newcommand\textSMC[1]{{\SMC #1}}
\newcommand\acro[1]{\textSMC{#1}\@}

\makeatother

% command for vectors
\newcommand{\bv}[1]{\ensuremath{\vec{#1}}}
% command for unit vectors
\newcommand{\uv}[2][blank]{%
\ifthenelse{\equal{#1}{blank}}%
{\ensuremath{\hat{u}_{#2}}}%
{}%
%
\ifthenelse{\equal{#1}{.}}%
{\ensuremath{\dot{\hat{u}}_{#2}}}%
{}%
%
\ifthenelse{\equal{#1}{'}}%
{\ensuremath{\hat{u}'_{#2}}}%
{}%
}
\newcommand{\ui}{\ensuremath{\hat{\imath}}}
\newcommand{\uj}{\ensuremath{\hat{\jmath}}}
\newcommand{\uk}{\ensuremath{\hat{k}}}

